AudioBERT: Audio Knowledge Augmented Language Model

Recent studies have identified that language models, pretrained on text-only datasets, often lack elementary visual knowledge, \textit{e.g.,} colors of everyday objects. Motivated by this observation, we ask whether a similar shortcoming exists in terms of the \textit{auditory} knowledge. To answer this question, we construct a new dataset called AuditoryBench, which consists of two novel tasks for evaluating auditory knowledge. Based on our analysis using the benchmark, we find that language models also suffer from a severe lack of auditory knowledge. To address this limitation, we propose AudioBERT, a novel method to augment the auditory knowledge of BERT through a retrieval-based approach. First, we detect auditory knowledge spans in prompts to query our retrieval model efficiently. Then, we inject audio knowledge into BERT and switch on low-rank adaptation for effective adaptation when audio knowledge is required. Our experiments demonstrate that AudioBERT is quite effective, achieving superior performance on the AuditoryBench. The dataset and code are available at \bulurl{https://github.com/HJ-Ok/AudioBERT}.

==> table/table1.tex <==
\begin{table}[t]
\caption{Audio sound recognition accuracy based on Wikipedia animal onomatopoeia data.} 
\centering
\vspace{0.25cm}
\resizebox{0.45\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
 Model & Top-1 & Top-5   \\ \midrule
BERT-base & 3.05 & 12.18 \\
BERT-large & 5.58 & 14.21  \\
Gemma2-2B & 6.60 & 16.75  \\
Llama3.1-8B & 16.24 & 26.40  \\
\bottomrule
\end{tabular}%
}
\label{tab:language_performance_in_animal_sound}
\end{table} 





% 

==> table/table6.tex <==
\begin{table}[t]
\caption{Statistics for sound pitch comparison Data}
\centering
\vspace{0.25cm}
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{lccc}
\hline
\textbf{Splits} & \textbf{\# Captions} & \textbf{\# Words/Caption} & \textbf{\# Total tokens}  \\ \hline
Train & 8,312 & 18.18 & 151,081  \\ 
Dev & 1,178 & 18.12 & 21,343  \\ 
Test & 2,387 & 18.19 & 43,431  \\ \hline
Total & 11,877 & 18.17 & 215,855  \\ \hline
\end{tabular}
}
\label{tab:height_of_sound}
\end{table}

